Disrupting Vision-Language Model-Driven Navigation Services via Adversarial Object Fusion

We present Adversarial Object Fusion (AdvOF), a novel attack framework targeting vision-and-language navigation (VLN) agents in service-oriented environments by generating adversarial 3D objects. While foundational models like Large Language Models (LLMs) and Vision Language Models (VLMs) have enhanced service-oriented navigation systems through improved perception and decision-making, their integration introduces vulnerabilities in mission-critical service workflows. Existing adversarial attacks fail to address service computing contexts, where reliability and quality-of-service (QoS) are paramount. We utilize AdvOF to investigate and explore the impact of adversarial environments on the VLM-based perception module of VLN agents. In particular, AdvOF first precisely aggregates and aligns the victim object positions in both 2D and 3D space, defining and rendering adversarial objects. Then, we collaboratively optimize the adversarial object with regularization between the adversarial and victim object across physical properties and VLM perceptions. Through assigning importance weights to varying views, the optimization is processed stably and multi-viewedly by iterative fusions from local updates and justifications. Our extensive evaluations demonstrate AdvOF can effectively degrade agent performance under adversarial conditions while maintaining minimal interference with normal navigation tasks. This work advances the understanding of service security in VLM-powered navigation systems, providing computational foundations for robust service composition in physical-world deployments.

==> body/algorithm.tex <==
%<*view>
\begin{algorithm}[t]
    \caption{Adversarial Object Fusion.}
    \DontPrintSemicolon
    \label{alg_viw}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$ T, \mathcal{V}, \mathcal{R},  Max$}
    \Output{$C^{adv}$}
    $(\text{MASK}, \text{SCORE}) \leftarrow \text{Object segmentation via Eq. 3}$\;
    $O \leftarrow \text{Object alignment via Eq. 4}$\;
    $\delta^{adv} \leftarrow \text{Initialize the 3D adversarial perturbation}$\;
    \For{$v\in\mathcal{V}$}{
        $w_{v}\xleftarrow{v}\mathcal{W}, mask_{v}\xleftarrow{v}MASK$\;
        \For{k in Max}{
            \tcp{Local Update}
            \textbf{Render}: $\delta^{adv}_{v} \leftarrow \mathcal{R}(\delta^{adv}, v)$\;
            \textbf{Optimize}: collaborative optimization via Eq. 18\;
            \textbf{Update}: $\delta^{adv} \xleftarrow{w_{v}} \delta^{adv}_{v}$\;
            \tcp{Consistency Determination}
            Judge the update for $v-1$ with $w_v$\;
            \tcp{Fusion Determination}
            Judge the perception for $v-1$\;
        }
    }
    $O^{adv}\leftarrow O+\delta^{adv}$\;
    return $C^{adv}$\;
\end{algorithm}
%</view>

==> body/figure.tex <==
%<*intro>
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{body/figure/intro.pdf}
    \caption{Attacking a VLN agent with the adversarial object. The VLN Agent misidentifies the adversarial object (original ``chair'')  as the fire extinguisher.}
    \label{fig:intro}
\end{figure}
%</intro>

%<*problem>
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{body/figure/problem.pdf}
    \caption{Vision-and-Language navigation agents with adversarial environment.}
    \label{fig:problem}
\end{figure*}
%</problem>

%<*method>
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{body/figure/method.pdf}
    \caption{Pipeline for generating adversarial environment towards VLN agents: It optimizes the adversarial object, transforming a normal environment into an adversarial one. \textit{Aligned object rendering} aligns the victim object in both 2D and 3D locations, rendering 2d images across different views. \textit{Collaborative optimization} jointly matches features between the adversarial and victim objects across 2D and 3D spaces. \textit{Adversarial object fusion} assigns importance weights to different views, contributing to generate adaptable adversarial object.
    }
    \label{fig:method}
\end{figure*}
%</method>

%<*example>
\begin{figure*}[t]
    \centering
    \subfigure[No Attack]{
        \begin{minipage}[t]{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/method/clean.pdf}
            \label{fig:examplea}
        \end{minipage}%
    }
    \subfigure[$\mathcal{L}_{I2I}$]{
        \begin{minipage}[t]{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/method/whole.pdf}
            \label{fig:exampleb}
        \end{minipage}
    }
    \subfigure[$\mathcal{L}_{2D}^{T}$ w/o $\mathcal{L}^{I2T}$]{
        \begin{minipage}[t]{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/method/no_text.pdf}
            \label{fig:examplec}
        \end{minipage}
    }
    \subfigure[$\mathcal{L}_{2D}^{T}$ w/o $\mathcal{L}^{B2B}$]{
        \begin{minipage}[t]{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/method/no_back.pdf}
            \label{fig:exampled}
        \end{minipage}
    }
    \subfigure[$\mathcal{L}_{2D}^{T}$]{
        \begin{minipage}[t]{0.19\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/method/all.pdf}
            \label{fig:examplee}
        \end{minipage}
    }
    \caption{Visualization of optimization results under different regularization terms for the target attack (table $\rightarrow$ alarm).}
    \label{fig:example}
\end{figure*}

%</example>

%<*simulator>
\begin{figure}[t]
    \centering
    \subfigure[MP3D, ID=5LpN3gDmAk7]{
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth, trim=0 0 0 215px, clip]{body/figure/experiment/scene/mp3d.png}
            \label{fig:mp3d}
        \end{minipage}
    }
    \hfill
    \subfigure[HM3D, ID=QaLdnwvtxbs]{
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/experiment/scene/hp3d.png}
            \label{fig:hm3d}
        \end{minipage}
    }
    \caption{The scene displayed on the habitat simulator.}
    \label{fig:simulator}
\end{figure}
%</simulator>

%<*noise>
\begin{figure}[t]
    \centering
    \subfigure[\scriptsize No attack (chair=0.44)]{
        \begin{minipage}[t]{0.3\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/experiment/delta/clean.png}
            \label{fig:noise_clean}
        \end{minipage}%
    }
    \hfill
    \subfigure[\scriptsize MF (chair=0.41)]{
        \begin{minipage}[t]{0.3\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/experiment/delta/mf.png}
            \label{fig:noise_mf}
        \end{minipage}%
    }
    \hfill
    \subfigure[\scriptsize AdvCLIP (chair=0.13)]{
        \begin{minipage}[t]{0.3\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/experiment/delta/advclip.png}
            \label{fig:noise_advclip}
        \end{minipage}%
    }
    \par
    \subfigure[\scriptsize ST (table=0.33)]{
        \begin{minipage}[t]{0.3\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/experiment/delta/st.png}
            \label{fig:noise_st}
        \end{minipage}%
    }
    \hfill
    \subfigure[\scriptsize TT3D (table=0.54)]{
        \begin{minipage}[t]{0.3\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/experiment/delta/tt3d.png}
            \label{fig:noise_tt3d}
        \end{minipage}%
    }
    \hfill
    \subfigure[\scriptsize AdvOF (table=0.81)]{
        \begin{minipage}[t]{0.3\linewidth}
            \centering
            \includegraphics[width=\textwidth]{body/figure/experiment/delta/advof.png}
            \label{fig:noise_advof}
        \end{minipage}%
    }
    \caption{The adversarial examples visualization of different attacks (chair $\rightarrow$ table).}
    \label{fig:noise}
\end{figure}
%</noise>

%<*view>
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{body/figure/experiment/multi_view.pdf}
    \caption{The adversarial object of different views. TV(black) $\rightarrow$ alarm(red).}
    \label{fig:view}
\end{figure}
%</view>

%<*epsilon>
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{body/figure/experiment/epsilon.pdf}
    \caption{Attacking results of different upper bounds.}
    \label{fig:epsilon}
\end{figure}
%</epsilon>

%<*goal>
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{body/figure/experiment/goals.pdf}
    \caption{Attacking results of different subordinate goals.}
    \label{fig:goal}
\end{figure}
%</goal>

%<*resilience>
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{body/figure/experiment/multi_noise.pdf}
    \caption{The attacking results of the adversarial object against to different noise. fridge (black) $\rightarrow$ knife (red)}
    \label{fig:resilience}
\end{figure*}
%</resilience>

==> body/table.tex <==
%<*simulator>
\begin{table}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{The setups of different VLN agents.}
    \setlength{\tabcolsep}{2.0mm}{%
    \begin{tabular}{llccc}
        \toprule
        \textbf{Agent}    & \textbf{Publication}              & \textbf{Simulator} & \textbf{Dataset} & {VLM} \\ \midrule
        Vlmaps~\cite{huang2023visual}               & ICRA'23                  & Habitat   & MP3D~\cite{chang2017matterport3d}   & Lseg~\cite{li2022languagedriven}   \\
        Cow~\cite{gadre2023cows}   & CVPR'23           & Habitat   & MP3D~\cite{chang2017matterport3d} & Clip~\cite{radford2021learning}      \\
        CF~\cite{shafiullahclip}   & RSS'23           & Habitat   & HM3D~\cite{ramakrishnan2021habitatmatterport} & Clip~\cite{radford2021learning}      \\
        ORION~\cite{dai2023think}                & ICRA'24             & Habitat   & HM3D~\cite{ramakrishnan2021habitatmatterport}   & Lseg~\cite{li2022languagedriven}   \\ \bottomrule
    \end{tabular}}
    \label{tab:simulator}
\end{table}
%</simulator>

%<*instruction> 
\begin{table}[t]
    \centering
    \footnotesize
    \renewcommand\arraystretch{1.2}
    \caption{The instruction samples of different VLN agents.}
    \begin{tabularx}{\columnwidth}{l|X}
        \toprule
        \textbf{Agents}     & \textbf{Instruction} \\ \midrule
        Vlmaps     & Go to the closest cushion first, then go to a chair nearby, after that, go to a counter and in the end, navigate to a table. \\
        \hdashline
        Cow        & Find a house plant near a coffee table. \\
        \hdashline
        CF         & A comfy place to sit and watch tv. \\
        \hdashline
        ORION      & Can you find a blue tower for me? It's hanging on the bar in the bathroom.  \\ \bottomrule
    \end{tabularx}
    \label{tab:instruction}
\end{table}
%</instruction>

%<*overall>
\begin{table*}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{
    The overall attacking performance of different methods on various VLN agents. 
    The upper and bottom parts respectively show the performance with and without attack objects. 
    }
    \setlength{\tabcolsep}{1.7mm}{%
    \begin{tabular}{llcccccccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Environment}}&\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Vlmaps}} & \multicolumn{3}{c}{\textbf{Cow}} & \multicolumn{3}{c}
        {\textbf{CF}} & \multicolumn{3}{c}{\textbf{ORION}} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
                              &  & \textbf{KPA} $\downarrow$           & \textbf{SPL} $\uparrow$    & \textbf{SR} $\downarrow$      & \textbf{KPA} $\downarrow$               & \textbf{SPL} $\uparrow$      & \textbf{SR} $\downarrow$      & \textbf{KPA} $\downarrow$                & \textbf{SPL} $\uparrow$      & \textbf{SR} $\downarrow$      & \textbf{KPA} $\downarrow$    & \textbf{SPL} $\uparrow$        & \textbf{SR} $\downarrow$        \\ \bottomrule
         \multirow{5}{*}{\textbf{Attacked}}&Base  & 0.560        & 49.0     & 0.297    & 0.208           & 12.6      & 0.158      & 0.275            & 17.2      & 0.198      & 0.215        & 9.8     & 0.147    \\
         \cdashline{2-14}
        &MF~\cite{zhao202evaluating}                      & 0.504        & 53.9   &  0.267      & 0.187           & 13.9     & 0.142       &  0.252                & 18.9      & 0.178         & 0.190        & 10.8     & 0.135   \\
        &AdvCLIP~\cite{zhou2023advclip}                 & 0.448        & 58.5   & 0.240      & 0.165           & 14.9   & 0.127         & 0.225                 & 20.3       & 0.162          & 0.171        & 11.7   & 0.115     \\
        &ST~\cite{liu2020spatiotemporal}                 & 0.392        & 64.0   & 0.208      & 0.148           & 16.2   & 0.109         & 0.193                 & 22.0       & 0.138          & 0.149        & 12.7   & 0.105     \\
        &TT3D~\cite{huang2024towards}                 & 0.331        & 67.8   & 0.184      & 0.125           & 17.7   & 0.096         & 0.163                 & 24.2       & 0.117          & 0.125        & 13.8   & 0.087     \\
        &\method{}(Untargeted)                & \underline{0.283}        & \underline{74.5}   & \underline{0.145}      & \underline{0.106}           & \underline{18.9}   & \underline{0.078}         & \underline{0.142}                 & \underline{25.8}        & \underline{0.102}        & \underline{0.104}        & \underline{14.9}   & \underline{0.072}     \\ 
        &\method{}(Targeted)                & \textbf{0.242}        & \textbf{77.5}    & \textbf{0.122}     & \textbf{0.084}            & \textbf{19.9}  & \textbf{0.067}         &  \textbf{0.116}       &   \textbf{27.0}   & \textbf{0.087}       & \textbf{0.089}       & \textbf{15.6}    & \textbf{0.064}    \\ \midrule
        & & \textbf{KPA} $\uparrow$           & \textbf{SPL} $\downarrow$   & \textbf{SR} $\uparrow$       & \textbf{KPA} $\uparrow$               & \textbf{SPL} $\downarrow$     & \textbf{SR} $\uparrow$         & \textbf{KPA} $\uparrow$                & \textbf{SPL} $\downarrow$     & \textbf{SR} $\uparrow$         & \textbf{KPA} $\uparrow$            & \textbf{SPL} $\downarrow$    & \textbf{SR} $\uparrow$      \\ \midrule
       \multirow{5}{*}{\textbf{Normal}} & Base                    & 0.480        & 58.0   & 0.218      & 0.192           & 17.3    & 0.114        & 0.251            & 21.2    & 0.157        & 0.204        & 11.7    & 0.121     \\
       \cdashline{2-14}
       & MF~\cite{zhao202evaluating}                 &  0.404       &  67.1   & 0.187      &  0.161        &      20.0     & 0.099  &   0.217               &   24.1        & 0.131      & 0.176         & 13.4     & 0.104    \\
       &  AdvCLIP~\cite{zhou2023advclip}                     &   \underline{0.475}      & 59.2   & \underline{0.214}      &   0.188         &   17.6      & 0.110   &      0.241           & \underline{21.5}     & 0.153          &  \underline{0.199}       & \underline{11.7}    & 0.119     \\
       &ST~\cite{liu2020spatiotemporal}                 & 0.442        & 61.9   & 0.209      & 0.177           & 18.4   & 0.107         & 0.235                 & 22.8       & 0.145          & 0.195        & 12.3  & 0.113     \\
        &TT3D~\cite{huang2024towards}                 & 0.437        & 61.7   & 0.205      & 0.174           & 18.4   & 0.103         & 0.232                 & 22.7       & 0.144          & 0.187        & 12.7   & 0.112     \\
       & \method{}(UnTargeted)          &  0.472             & \underline{58.2}      & 0.213        &  \underline{0.189}     & \underline{17.4}      & \underline{0.112}         &  \underline{0.248}          &  21.8     &  \underline{0.152}        & 0.197          & 11.9    & \underline{0.120}     \\ 
      &  \method{}(Targeted)                &  \textbf{0.480}      & \textbf{58.0}     & \textbf{0.218}     &    \textbf{0.190}       &  \textbf{17.1}   & \textbf{0.115}      &   \textbf{0.251}              & \textbf{21.2}    & \textbf{0.156}      &  \textbf{0.202}      &   \textbf{11.6}  & \textbf{0.122}    \\\bottomrule
    \end{tabular}}
    \label{tab:overall}
\end{table*}
%</overall>


%<*clean>
\begin{table*}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{The overall performance results for clean datasets of different attacking methods on various VLN agents.}
    \setlength{\tabcolsep}{2.5mm}{%
    \begin{tabular}{lcccccccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Vlmaps}} & \multicolumn{3}{c}{\textbf{Cow(PASTURE)}} & \multicolumn{3}{c}
        {\textbf{Cow(RoboTHOR)}} & \multicolumn{3}{c}{\textbf{ORION}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
                                & \textbf{KPA} $\uparrow$           & \textbf{SPL} $\downarrow$   & \textbf{SR} $\uparrow$       & \textbf{KPA} $\uparrow$               & \textbf{SPL} $\downarrow$     & \textbf{SR} $\uparrow$         & \textbf{KPA} $\uparrow$                & \textbf{SPL} $\downarrow$     & \textbf{SR} $\uparrow$         & \textbf{KPA} $\uparrow$            & \textbf{SPL} $\downarrow$    & \textbf{SR} $\uparrow$      \\ \bottomrule
        \rowcolor{lightgreen}
        Base                    & 0.480        & 58.0   & 0.218      & 0.192           & 17.3    & 0.114        & 0.251            & 21.2    & 0.157        & 0.204        & 11.7    & 0.121     \\
        \hdashline
        MF~\cite{zhao202evaluating}                      &   0.271      & 104.5   & 0.134      &   0.109         &   36.4      & 0.073   &      0.127           & 74.7     & 0.084          &  0.105       & 48.3    & 0.059     \\
        AdvCLIP~\cite{zhou2023advclip}                 &  0.410       &  65.5   & 0.184      &  0.156        &      25.1     & 0.098  &   0.196               &   44.3        & 0.123      & 0.195         & 13.5     & 0.087    \\
        \rowcolor{lightred!50} 
        
        \rowcolor{lightred!50}
        Ours(UnTargeted)                &              &       &         &                 &       &         &                &      &         &   -           &    -    & -    \\ 
        Ours(Targeted)                &  0.432      & 60.7     & 0.171     &    0.149       &  28.4   & 0.087      &   0.185              & 50.7    & 0.104      &  0.173      &   21.6  & 0.081    \\ 
        \bottomrule
    \end{tabular}}
    \label{tab:clean}
\end{table*}
%</clean>

%<*labelacc>
\begin{table}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{
    Attacking results towards perception modules across different VLN agents.
    }
    \setlength{\tabcolsep}{2.0mm}{\begin{tabular}{lllllllll}
        \toprule
            & \multicolumn{2}{c}{\textbf{Vlmaps}} & \multicolumn{2}{c}{\textbf{Cow}} & \multicolumn{2}{c}{\textbf{CF}} & \multicolumn{2}{c}{\textbf{ORION}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
            & \textbf{Acc}          & \textbf{Asr}         & \textbf{Acc}        & \textbf{Asr}        & \textbf{Acc}        & \textbf{Asr}       & \textbf{Acc}         & \textbf{Asr}         \\  \midrule
    Base    & 0.89         & 0.00        & 0.83       & 0.00       & 0.81       & 0.00      & 0.91        & 0.00        \\
    \hdashline
    MF      & 0.71         & 0.15        & 0.74       & 0.06       & 0.69       & 0.12      & 0.83        & 0.08        \\
    AdvCLIP & 0.56         & 0.34        & 0.60       & 0.32       & 0.61       & 0.35      & 0.68        & 0.26        \\
    ST      & 0.33         & 0.56        & 0.27       & 0.61       & 0.30       & 0.64      & 0.29        & 0.65        \\
    TT3D    & 0.29         & 0.70        & 0.21       & 0.76       & 0.20       & 0.78      & 0.26        & 0.71        \\
    \method{}   & \textbf{0.04}         & \textbf{0.92}        & \textbf{0.05}       & \textbf{0.91}       & \textbf{0.02}       & \textbf{0.93}      & \textbf{0.05}        & \textbf{0.94} \\\bottomrule       
    \end{tabular}}
    \label{tab:label}
\end{table}
%</labelacc>

%<*sizetransfer>
\begin{table}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{Results of transfer attack across different image encoders.}
    \setlength{\tabcolsep}{0.7mm}{\begin{tabular}{llll}
        \toprule
          & \textbf{KPA} $\downarrow$           & \textbf{SPL} $\uparrow$   & \textbf{SR} $\downarrow$ \\\midrule
        \multirow{2}{*}{Lseg, ViT-L/16 $\rightarrow$ Lseg, ResNet101} & 0.242   & 77.5    & 0.122  \\
        & 0.287(\textcolor{red}{18.6\%})    & 73.2(\textcolor{red}{5.6\%})    & 0.147(\textcolor{red}{20.5\%})  \\
        \hdashline
        \multirow{2}{*}{Lseg, ResNet101 $\rightarrow$ Lseg, ViT-L/16}  & 0.253   & 76.8   & 0.134  \\
        & 0.302(\textcolor{red}{19.4\%})   & 70.1(\textcolor{red}{8.7\%})   & 0.163(\textcolor{red}{21.6\%})  \\
        \hdashline
        \multirow{2}{*}{Clip, ViT-B/32 $\rightarrow$ Clip, ViT-L/16} & 0.084   & 19.9    & 0.067  \\
        & 0.105(\textcolor{red}{25.0\%})   & 19.0(\textcolor{red}{4.5\%})    & 0.076(\textcolor{red}{13.4\%})  \\
        \hdashline
        \multirow{2}{*}{Clip, ViT-L/16 $\rightarrow$ Clip, ViT-B/32} & 0.095   & 19.4   & 0.072 \\
        & 0.092(\textcolor{red}{3.1\%})   & 19.4(\textcolor{red}{0.0\%})   & 0.073(\textcolor{red}{1.4\%}) \\
        \bottomrule
    \end{tabular}}
    \label{tab:sizetransfer}
\end{table}
%</sizetransfer>

%<*datatransfer>
\begin{table}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{Results of transfer attack across different datasets.}
    \begin{tabular}{lccc}
        \toprule
      & \textbf{KPA} $\downarrow$           & \textbf{SPL} $\uparrow$   & \textbf{SR} $\downarrow$ \\\midrule
    \multirow{2}{*}{MP3D1 $\rightarrow$ MP3D2} & 0.242   & 77.5   & 0.122  \\
    & 0.254(\textcolor{red}{5.0\%})  & 75.8(\textcolor{red}{2.2\%})   & 0.128(\textcolor{red}{4.9\%})  \\
    \hdashline
    \multirow{2}{*}{MP3D2 $\rightarrow$ MP3D1} & 0.253   & 75.1   & 0.132  \\
    & 0.257(\textcolor{red}{1.6\%})   & 75.5(\textcolor{green}{0.5\%})   & 0.133(\textcolor{red}{0.8\%})  \\
    \hdashline
    \multirow{2}{*}{HM3D1 $\rightarrow$ HM3D2} & 0.089   & 15.6   & 0.064  \\
    & 0.096(\textcolor{red}{7.9\%})   & 15.1(\textcolor{red}{3.3\%})   & 0.069(\textcolor{red}{7.8\%})  \\
    \hdashline
    \multirow{2}{*}{HM3D2 $\rightarrow$ HM3D1}  & 0.100   & 18.8   & 0.076  \\
    & 0.104(\textcolor{red}{4.0\%})   & 18.0(\textcolor{red}{4.4\%})   & 0.081(\textcolor{red}{6.6\%})  \\
    \bottomrule
    \end{tabular}
    \label{tab:datatransfer}
\end{table}
%</datatransfer>

%<*modeltransfer>
\begin{table}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{Results of transfer attack across different models.}
    \begin{tabular}{lccc}
        \toprule
      & \textbf{KPA} $\downarrow$           & \textbf{SPL} $\uparrow$   & \textbf{SR} $\downarrow$ \\\midrule
    \multirow{2}{*}{(Lseg) $\rightarrow$ (Clip)} & 0.084   & 19.9   & 0.067  \\
    & 0.125   & 17.7   & 0.096  \\
    & 0.131(\textcolor{red}{4.8\%})   & 17.2(\textcolor{red}{2.9\%})   & 0.097(\textcolor{red}{1.0\%})  \\
    \hdashline
    \multirow{2}{*}{(Clip)$\rightarrow$ (Lseg)} & 0.242   &  77.5  & 0.122  \\
    & 0.331   &  67.8  & 0.184  \\
    & 0.313(\textcolor{green}{5.4\%})   &  71.9(\textcolor{green}{6.0\%})  & 0.159(\textcolor{green}{13.4\%})  \\
    \bottomrule
    \end{tabular}
    \label{tab:modeltransfer}
\end{table}
%</modeltransfer>

%<*transfer>
\begin{table*}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{Results of transfer attack against to white-box VLN agents.}
    \setlength{\tabcolsep}{2.5mm}{%
    \begin{tabular}{lcccccccccccc}
    \toprule
     \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{l}{\textbf{Vlmaps (Lseg, ViT-L/16)}} & \multicolumn{3}{l}{\textbf{Cow(Clip, ViT-B/32)}} & \multicolumn{3}{l}{\textbf{Cow(Clip, ViT-B/32)}} & \multicolumn{3}{l}{\textbf{ORION(Lseg, ViT-L/16)}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
                                & \textbf{KPA} $\uparrow$           & \textbf{SPL} $\downarrow$   & \textbf{SR} $\uparrow$       & \textbf{KPA} $\uparrow$               & \textbf{SPL} $\downarrow$     & \textbf{SR} $\uparrow$         & \textbf{KPA} $\uparrow$                & \textbf{SPL} $\downarrow$     & \textbf{SR} $\uparrow$         & \textbf{KPA} $\uparrow$            & \textbf{SPL} $\downarrow$    & \textbf{SR} $\uparrow$      \\ \bottomrule
    LSeg (ResNet101) &               &              &              &             &             &             &             &             &             &              &              &             \\
    LSeg (ViT-L/16)  &               &              &              &             &             &             &             &             &             &              &              &             \\
    Clip (ViT-B/16)  &               &              &              &             &             &             &             &             &             &              &              &             \\
    Clip (ViT-B/32)  &               &              &              &             &             &             &             &             &             &              &              &    \\\bottomrule         
    \end{tabular}}
    \label{tab:transfer}
\end{table*}
%</transfer>

%<*physicalnoise>
\begin{table}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{Results of physical noise against to adversarial objects.}
    \setlength{\tabcolsep}{5mm}{\begin{tabular}{llll}
        \toprule
                    & KPA $\downarrow$  & SPL $\uparrow$  & SR $\downarrow$  \\\midrule
        Clean       & 0.560     & 49.0     & 0.297   \\
        \method{}      & 0.242     & 77.5     & 0.122   \\
        \hdashline
        with Shear       & 0.283   & 74.1    & 0.149   \\
        with Scaling     & 0.255    & 76.5    &  0.132  \\
        with Gaussian    & 0.289    & 72.1   &  0.150  \\
        with Brightness+ & 0.243    & 75.2    & 0.138   \\
        with Brightness- & 0.241   & 75.0    & 0.129  \\
        \bottomrule
    \end{tabular}}
    \label{tab:physicalnoise}
\end{table}
%</physicalnoise>

%<*budget>
\begin{table}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{Results of different perturbation upper bound.}
    \setlength{\tabcolsep}{5mm}{%
    \begin{tabular}{lccc}
    \toprule
     Budget & \textbf{KPA} $\uparrow$           & \textbf{SPL} $\downarrow$   & \textbf{SR} $\uparrow$  \\ \midrule
    $\epsilon=0.01$  &   0.283            &   65.6           &    0.175         \\
    $\epsilon=0.02$  &   0.276            &    66.7         &    0.168         \\
    $\epsilon=0.03$  &   0.265            &    68.3          &    0.165          \\
    $\epsilon=0.04$  &   0.254            &   68.9           &    0.159          \\
    $\epsilon=0.05$  &   0.252            &   69.3           &  0.157         \\\bottomrule         
    \end{tabular}}
    \label{tab:budget}
\end{table}
%</budget>

%<*object>
\begin{table}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{Results of different target object selection.}
    \setlength{\tabcolsep}{5mm}{%
    \begin{tabular}{lccc}
        \toprule
        & KPA & SPL & SR \\\midrule
        sub-goal@1 & -   & -   & -  \\
        sub-goal@2 & -   & -   & -  \\
        sub-goal@3 & -   & -   & -  \\
        sub-goal@4 & -   & -   & - \\\bottomrule
    \end{tabular}}
    \label{tab:object}
\end{table}
%</object>

%<*ablation>
\begin{table}[t]
    \centering
    \renewcommand\arraystretch{1.2}
    \footnotesize
    \caption{Results of Ablation Study.}
    \setlength{\tabcolsep}{5mm}{%
    \begin{tabular}{lccc}
        \toprule
        & \textbf{KPA} $\downarrow$ & \textbf{SPL} $\uparrow$ & \textbf{SR} $\downarrow$ \\\midrule
        \method{} & 0.242   & 77.5   & 0.122  \\
        w/o $Alignment$ & 0.450   & 59.6   & 0.233  \\
        w/o $\mathcal{L}_{2d}$ & 0.512   & 53.5   & 0.267  \\
        w/o $\mathcal{L}_{3d}$ & 0.310   & 70.1   & 0.169  \\
        w/o $Fusion$ & 0.338   & 68.9   & 0.176 \\\bottomrule
    \end{tabular}}
    \label{tab:ablation}
\end{table}
%</ablation>

%<*robustness>
\begin{table}[t]
    \centering
    \renewcommand\arraystretch{1.0}
    \footnotesize
    \caption{Agent robustness in scenes with different noises.}
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{lcccccc}
        \toprule
         & \multicolumn{3}{c}{Adv} & \multicolumn{3}{c}{Gaussian} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
         & \textbf{KPA} $\uparrow$           & \textbf{SPL} $\downarrow$   & \textbf{SR} $\uparrow$ & \textbf{KPA} $\uparrow$           & \textbf{SPL} $\downarrow$   & \textbf{SR} $\uparrow$ \\ \midrule
    Base &  -       &    -            & -           &  -                 & -             &  -           \\
    GT   &  -       &    -            & -           &  -                 & -             &  -           \\
    AT   &  -       &    -            & -           &  -                 & -             &  -           \\ \bottomrule          
    \end{tabular}}
    \label{tab:robustness}
\end{table}
%</robustness>
